RESPECT: Reinforcement Learning based Edge Scheduling on Pipelined Coral Edge TPUs

Deep neural networks (DNNs) have substantial computational and memory requirements, and the compilation of its computational graphs has a great impact on the performance of resource-constrained (e.g., computation, I/O, and memory-bound) edge computing systems. While efficient execution of their computational graph requires an effective scheduling algorithm, generating the optimal scheduling solution is a challenging NP-hard problem. Furthermore, the complexity of scheduling DNN computational graphs will further increase on pipelined multi-core systems considering memory communication cost, as well as the increasing size of DNNs. Using the synthetic graph for the training dataset, this work presents a reinforcement learning (RL) based scheduling framework RESPECT, which learns the behaviors of optimal optimization algorithms and generates near-optimal scheduling results with short solving runtime overhead. Our framework has demonstrated up to $\sim2.5\times$ real-world on-chip inference runtime speedups over the commercial compiler with ten popular ImageNet models deployed on the physical Coral Edge TPUs system. Moreover, compared to the exact optimization methods, the proposed RL scheduling improves the scheduling optimization runtime by up to 683$\times$ speedups compared to the commercial compiler and matches the exact optimal solutions with up to 930$\times$ speedups. Finally, we perform a comprehensive generalizability test, which demonstrates RESPECT successfully imitates optimal solving behaviors from small synthetic graphs to large real-world DNNs computational graphs.

==> 05-sec-power-results.tex <==
%\subsection{Energy Efficiency Evaluation}
%\label{sec:edgetpu_energy}








% \begin{figure*}[h]
%     \centering
% \begin{subfigure}[b]{1\textwidth}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/Energy.pdf}
%     \caption{4,5,6-stage pipelined Edge TPUs energy efficiency comparisons between RL methods and commercial Edge TPU compiler which demonstrates the energy efficiency improvement of RESPECT framework. Overall, RL methods has a power efficiency improvement of $25.5\%$.}
%     \label{fig:power_results}
% \end{subfigure}

% \begin{subfigure}[b]{1\textwidth}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/memory.pdf}
%     \caption{Memory allocation for all models between RL methods and commercial Edge TPU compiler. Evenly }
%     \vspace{-3mm}
%     \label{fig:memory}
% \end{subfigure}
% \caption{Memory and energy efficiency comparison between 4,5,6 stages}
% \label{fig:energy/memory}
% \end{figure*}


\noindent
\textbf{Energy efficiency} -- Besides, we compare the energy efficiency between RESPECT and commercial Edge TPU compiler. We integrate the power meter of the AVHzY CT-3 USB 3.1 Power Meter\footnote{\url{www.avhzy.com}} into our power measurement system (Figure \ref{fig:power_measure_sys}). Power meter is attached with one single TPU and remaining TPUs are connected with host using a USB 3.0 hub and results are reported in Watt/frame/second (Watt/FPS). The power measurement results are shown in Figure \ref{fig:power_results}. 
%{\color{red} We can see that RESPECT has significant power efficiency improvement. Both of the better computation resource utilization and smaller communication cost together leads to power efficiency improvements. According to the 12 models we tests, RL scheduling methods has average energy efficiency improvement of 9.8\% (with up to 60.8\%), 25.5\% (with up to 59.4\%), and 20.9\% (with up to 66.8\%). For example, for model Xception in 5 stage system, the energy efficiency is improved over the heuristic methods, which reduces the power consumption for each framework inference from 6.35 $\times 10^{-2}$ Watt/FPS to 3.98 $\times 10^{-2}$ Watt/FPS (59.4\% improvement).} 
{RESPECT offers significant power efficiency improvements with the increased computation resource utilization and minimized communication costs together. Specifically, RESPECT scheduling improves energy efficiency improvement by 9.8\% in average for the 12 models (with up to 60.8\%), 25.4\% (with up to 59.4\%), and 20.9\% (with up to 66.8\%), in 4-, 5-, and 6-stage pipeline Edge TPU systems. For example, with ImageNet-Xception model in 5-stage system, the energy efficiency is improved from 6.35 $\times 10^{-2}$ Watt/FPS to 3.98 $\times 10^{-2}$ Watt/FPS (i.e., 59.4\% improvement), compared to commercial Edge TPU compiler.}

%From the analysis of runtime performance and energy efficiency in this two section, we can find some performance miscorrelation. Specially, some RL generated scheduling have better performance than exact methods. On the other hand, RL scheduling perform worse than Edge TPU compiler for model ResNet101. We have in-depth analysis in Section \ref{sec:memory}.

% {From the analysis of runtime performance and energy efficiency in these two sections, we observe that exact methods sometimes perform worse than RESPECT as well. This is due to the miscorrelation between the high-level abstract modeling of computational graphs and the actual systolic hardware specifications. %Specially, some RL generated scheduling have better performance than exact methods. On the other hand, RL scheduling perform worse than Edge TPU compiler for model ResNet101. 
% }

\noindent
{\textbf{Performance modeling miscorrelation} -- From the analysis of runtime performance and energy efficiency shown in {Figures \ref{fig:edgetpu_runtime} and \ref{fig:power_results},} we observe that exact methods sometimes perform worse than RESPECT. This is due to the miscorrelation between the high-level abstract modeling of computational graphs and the actual systolic hardware specifications, in which the hardware architecture and backend compilation are closed source. Such miscorrelations of the high-level performance modeling can be used to guide the scheduling optimizations but introduce optimization noise to the actual on-chip performance. Specifically, in this work, both the exact method and RESPECT optimize the DNN model scheduling from the aspects of the memory allocation and communication cost. Note that directly modeling or estimating the runtime from the computation graph and its schedule is impossible given the complexity of the Edge TPU compute components and caching/memory system \cite{boroumand2021mitigating,zhou2021rethinking}}.

\begin{figure*}[b]
    \centering
    \includegraphics[width=0.90\linewidth]{figures/speedup.pdf}
    \caption{Schedule solving time across ten real-world ImageNet models with different graph sizes. The horizontal-axis and vertical-axis represent graph sizes |V|, and speedups over the baselines, respectively. RL method offers $24-683\times$ speedups over Edge TPU compiler and $100-930\times$ over exact methods.}
    \label{fig:scheduling_overhead}
\end{figure*}


\vspace{-3mm}
\subsection{Solving Complexity and Generalizability} \label{sec:scheduling_overhead}

To demonstrate the robustness of our work, we demonstrate the solving complexity and generalizability of our work.

\noindent
{\textbf{Generalizability analysis--}} As we discussed before, the entire training process is fully conducted on synthetic graph sampling, where the training graph size is $|V|=30$ and the testing process is conducted with real-world DNN models. The experimental results shown in Table \ref{tbl:dnn_graphs} and Figure \ref{fig:edgetpu_runtime} also conclude the generalizability of the proposed approach. Specifically, as shown in Table \ref{tbl:dnn_graphs}, the sizes of the DNN computational graphs varies from $134$ to $782$, which are all far beyond the training graph $|V|=30$. Besides, the degree of the deployed DNNs models varies as well (e.g., $deg(V)=4$ in InceptionResNetv2 and $deg(V)=2$ in other models). The proposed RL framework consistently outperforms the commercial Edge TPU compiler in scheduling large computational graphs, even with the graph that is $26\times$ larger than the synthetic training samples ($|V|=782$ in InceptionResNetv2 versus $|V|=30$ in training).

\noindent
{\textbf{Solving complexity analysis--}} The previous section firstly demonstrates that the proposed RL approach significantly improves the scheduling solution over the Edge TPU compiler (heuristics) and has the same quality as the exact constraint solving scheduling method. Now, we will compare the schedule solving runtime of our proposed RL framework with the same baselines, to demonstrate the solving runtime complexity is simultaneously improved. %We empirically select 128 as the inference batch size. Because of our above-mention scheduling strategies in Section \ref{sec:approach}, the inference runtime is unstable for 4-stage, 5-stage, and 6-stage pipelining.
The solving runtime results are conducted on the same set of DNN models. For the exact method, we use IBM ILOG CPLEX to solve the constraint scheduling formulations. %The solving runtime represents the scheduling rumtime which is exponentially increased with the increasing of pipeline stages. For Edge TPU compiler, we analysis the compilation runtime and it is unstable for different pipeline stages.
{The results are shown in Figure \ref{fig:scheduling_overhead}, where the {horizontal-axis} represents the graph sizes, i.e, $|V|$ in the computation graph $G(V, E)$, the {vertical-axis} shows the speedup in solving runtime of the RL framework over the two baselines.}

%We can make two key observations for Figure \ref{fig:scheduling_overhead}: \textbf{(1) RL method cost much less solving runtime compared with other two methods.} RL can provide a speedup of $100\times$ to $930\times$ over exact method. Compared with Edge TPU compiler, RL provides speedups of $24\times$ to $683\times$; \textbf{(2) the speedup over exact method and Edge TPU compiler become smaller as graph size increases.} For example, scheduling of model InceptionResnetv2 (|V|=782) has a speedup of $100\times$,$296\times$,$270\times$ for 4-stage, 5-stage, and 6-stage, respectively. However, for Xception (|V| = 134), the speedup will reach up to $469\times$,$930\times$, and $782\times$, respectively. Thus, our proposed RL framework can provide a near-optimal inference runtime with much better scheduling scalability over Edge TPU compiler ($24\times$ to $683\times$) and exact methods ($100\times$ to $930\times$).

{Three important conclusions can be summarized from Figure \ref{fig:scheduling_overhead}: \textbf{(1) Compared to the heuristic methods (Edge TPU compiler), the main advantage of the proposed RL approach is the quality of scheduling in Edge TPU inference runtime.} Specifically, our RL approach offers $24\times$ to $683\times$ speedups over Edge TPU compiler, in generating the scheduling solutions, with up to 2.5$\times$ inference runtime improvements discussed in Section \ref{sec:edgetpu_runtime}. For example, for ResNet152, the RL generated schedule offers 2.4$\times$ speedups in Edge TPU inference runtime and simultaneously improves the scheduling solving time by 85$\times$. \textbf{(2) Compared to the exact method conducted on constraint solving scheduling, our RL approach offers $100\times$ to $930\times$ speedups in generating scheduling solutions, in which the Edge TPU inference runtime are almost identical}. For example, for the Xception model, the Edge TPU inference runtime is almost the same as RL approach and the exact method, but the RL scheduling solving time is 930$\times$ faster than the exact method. \textbf{(3) The scheduling solving time improvements decrease as the computation graph sizes $|V|$ increase.} As shown in Figure \ref{fig:scheduling_overhead}, there are clear trends that the speedups over both baselines decrease as the graph sizes increase. For example, scheduling of model InceptionResnetv2 (|V|=782) has a speedup of $100\times$, $296\times$, $270\times$ for 4-stage, 5-stage, and 6-stage pipelining, respectively. However, for Xception (|V| = 134), the speedup will reach up to $469\times$, $930\times$, and $782\times$, respectively. %Thus, our proposed RL framework can provide a near-optimal inference runtime with much better scheduling scalability over Edge TPU compiler ($24\times$ to $683\times$) and exact methods ($100\times$ to $930\times$).
}


 
\begin{figure*}[!htb]
     \centering
     \includegraphics[width=0.85\linewidth]{figures/memory.pdf}
     \caption{{Parameter caching analysis of 4-, 5-, 6-stage pipelined Edge TPUs systems for expainability of RESPECT RL, where RESPECT scheduling method decreases and balances the peak memory utilization for all models.% Note that off-chip memory dominates the runtime performance and energy efficiency which demonstrates the reason for performance improvement. 
     }
     \label{fig:memory_results}}
 \end{figure*}
 
{
\subsection{Parameter Caching Analysis for Explainablility of RESPECT}
\label{sec:memory}

To understand the runtime differences, we analyze the post-compiled execution graphs to extract explainable knowledge learned by the reinforcement process. Note that Edge TPU architecture is a template-based machine learning accelerator including a 2D array of processing elements (PE), where all PEs share memory over the core. In other words, while deploying the computation graph operators to the cores, it is critical to balance the memory and computation. In addition, for the multi-TPU pipelining with a central CPU host, the communication from stage to stage could significantly dominate the runtime performance, since it communicates via a slow I/O interface (e.g., USB 3.0). These have been confirmed by the two observations: (1) our RL model further optimizes the memory utilization for each stage (i.e., minimizing off-chip DRAM utilization and maximizing cache locality); (2) with more compute and memory resources (e.g., 6-stage), the communication cost becomes more critical since the models can be simply deployed with cache-only computation.

To demonstrate that RESPECT optimizes w.r.t memory caching, we provide a detailed parameter caching, as shown in Figure \ref{fig:memory_results}. It is well known that loading/storing parameters from off-cache memory is very time consuming. As shown in Edge TPU data-sheet \footnote{https://coral.ai/docs/accelerator/datasheet/}, coral USB accelerators have theoretical peak throughput of 2 TFLOP/s. Because Edge TPU performs INT8 operation, we can assume only 1 FLOPS/B performed. However, modern DRAM bandwidth (e.g., LPDDR4 has a bandwidth of 32 GB/s \cite{lpddr4}) is two orders of magnitude lower than 2 TB/s to sustain peak PE throughput. To optimize the parameter caching in Edge TPUs, we hope the input TFlite file should be evenly partitioned and each model file size should be less than 8MB.
We collect the maximum input parameter footprint sizes among all stages which are shown in Figure \ref{fig:memory_results}. We can see that our proposed RL scheduling has much smaller off-chip DRAM usage which is the main reason for runtime improvement. For example, model Resnet152 scheduled by RL methods (12.00 MB) with 5 stage system has smaller DRAM usage compared with Edge TPU compiler (13.95 MB). Hence, we can observe an energy efficiency improvement of $19.6\%$. From the memory analysis, we can see that evenly distributed memory helps to improve on-chip SRAM utilization and leads to better runtime performance. Overall, Our proposed RL scheduling methods decrease the peak memory utilization by 1.14\%, 13.5\%, and 2.2\% in 4-, 5-, and 6-stage pipeline Edge TPU systems.}

 
 
%\textbf{Explainable domain knowledge learned by RL--} 




==> bib.tex <==
\begin{thebibliography}{00}
\bibitem{Bengio+chapter2007}Bengio, Y. \& LeCun, Y. Scaling Learning Algorithms Towards AI. {\em Large Scale Kernel Machines}. (2007)
\bibitem{zhou2021rethinking}Zhou, Y., Dong, X., Akin, B., Tan, M., Peng, D., Meng, T., Yazdanbakhsh, A., Huang, D., Narayanaswami, R. \& Laudon, J. Rethinking co-design of neural architectures and hardware accelerators. {\em ArXiv Preprint ArXiv:2102.08619}. (2021)
\bibitem{chen2018tvm}Chen, T., Moreau, T., Jiang, Z., Zheng, L., Yan, E., Shen, H., Cowan, M., Wang, L., Hu, Y., Ceze, L. \& Others {TVM}: An automated end-to-end optimizing compiler for deep learning. {\em 13th {USENIX} Symposium On Operating Systems Design And Implementation ({OSDI} 18)}. pp. 578-594 (2018)
\bibitem{Hinton06}Hinton, G., Osindero, S. \& Teh, Y. A Fast Learning Algorithm for Deep Belief Nets. {\em Neural Computation}. \textbf{18} pp. 1527-1554 (2006)
\bibitem{goodfellow2016deep}Goodfellow, I., Bengio, Y., Courville, A. \& Bengio, Y. Deep learning. (MIT Press,2016)
\bibitem{hochreiter1997long}Hochreiter, S. \& Schmidhuber, J. Long short-term memory. {\em Neural Computation}. \textbf{9}, 1735-1780 (1997)
\bibitem{boroumand2021mitigating}Boroumand, A., Ghose, S., Akin, B., Narayanaswami, R., Oliveira, G., Ma, X., Shiu, E. \& Mutlu, O. Mitigating Edge Machine Learning Inference Bottlenecks: An Empirical Study on Accelerating Google Edge Models. {\em ArXiv Preprint ArXiv:2103.00768}. (2021)
\bibitem{yazdanbakhsh2021evaluation}Yazdanbakhsh, A., Seshadri, K., Akin, B., Laudon, J. \& Narayanaswami, R. An evaluation of edge tpu accelerators for convolutional neural networks. {\em ArXiv Preprint ArXiv:2102.10423}. (2021)
\bibitem{jouppi2017datacenter}Jouppi, N., Young, C., Patil, N., Patterson, D., Agrawal, G., Bajwa, R., Bates, S., Bhatia, S., Boden, N., Borchers, A. \& Others In-datacenter performance analysis of a tensor processing unit. {\em Proceedings Of The 44th Annual International Symposium On Computer Architecture}. pp. 1-12 (2017)
\bibitem{sheng2021deep}Sheng, S., Chen, P., Chen, Z., Wu, L. \& Yao, Y. Deep Reinforcement Learning-Based Task Scheduling in IoT Edge Computing. {\em Sensors}. \textbf{21}, 1666 (2021)
\bibitem{chen2019deep}Chen, H. \& Shen, M. A Deep-Reinforcement-Learning-Based Scheduler for FPGA HLS. {\em 2019 IEEE/ACM International Conference On Computer-Aided Design (ICCAD)}. pp. 1-8 (2019)
\bibitem{vaswani2017attention}Vaswani, A., Shazeer, N., Parmar, N., Uszkoreit, J., Jones, L., Gomez, A., Kaiser, Ł. \& Polosukhin, I. Attention is all you need. {\em Advances In Neural Information Processing Systems}. pp. 5998-6008 (2017)
\bibitem{williams1992simple}Williams, R. Simple statistical gradient-following algorithms for connectionist reinforcement learning. {\em Machine Learning}. \textbf{8}, 229-256 (1992)
\bibitem{bello2016neural}Bello, I., Pham, H., Le, Q., Norouzi, M. \& Bengio, S. Neural combinatorial optimization with reinforcement learning. {\em ArXiv Preprint ArXiv:1611.09940}. (2016)
\bibitem{chollet2017xception}Chollet, F. Xception: Deep learning with depthwise separable convolutions. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 1251-1258 (2017)
\bibitem{he2016identity}He, K., Zhang, X., Ren, S. \& Sun, J. Identity mappings in deep residual networks. {\em European Conference On Computer Vision}. pp. 630-645 (2016)
\bibitem{szegedy2017inception}Szegedy, C., Ioffe, S., Vanhoucke, V. \& Alemi, A. Inception-v4, inception-resnet and the impact of residual connections on learning. {\em Thirty-first AAAI Conference On Artificial Intelligence}. (2017)
\bibitem{he2016deep}He, K., Zhang, X., Ren, S. \& Sun, J. Deep residual learning for image recognition. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 770-778 (2016)
\bibitem{huang2017densely}Huang, G., Liu, Z., Van Der Maaten, L. \& Weinberger, K. Densely connected convolutional networks. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 4700-4708 (2017)
\bibitem{sanders2010cuda}Sanders, J. \& Kandrot, E. CUDA by example: an introduction to general-purpose GPU programming. (Addison-Wesley Professional,2010)
\bibitem{yu2018semantic}Yu, B., Yang, L. \& Chen, F. Semantic segmentation for high spatial resolution remote sensing images based on convolution neural network and pyramid pooling module. {\em IEEE Journal Of Selected Topics In Applied Earth Observations And Remote Sensing}. \textbf{11}, 3252-3261 (2018)
\bibitem{abadi2016tensorflow}Abadi, M., Barham, P., Chen, J., Chen, Z., Davis, A., Dean, J., Devin, M., Ghemawat, S., Irving, G., Isard, M. \& Others Tensorflow: A system for large-scale machine learning. {\em 12th {USENIX} Symposium On Operating Systems Design And Implementation ({OSDI} 16)}. pp. 265-283 (2016)
\bibitem{kuchcinski2003constraints}Kuchcinski, K. Constraints-driven scheduling and resource assignment. {\em ACM Transactions On Design Automation Of Electronic Systems (TODAES)}. \textbf{8}, 355-383 (2003)
\bibitem{lente2014exponential}Lenté, C., Liedloff, M., Soukhal, A. \& T'Kindt, V. Exponential algorithms for scheduling problems.  (2014)
\bibitem{mao2019learning}Mao, H., Schwarzkopf, M., Venkatakrishnan, S., Meng, Z. \& Alizadeh, M. Learning scheduling algorithms for data processing clusters. {\em Proceedings Of The ACM Special Interest Group On Data Communication}. pp. 270-288 (2019)
\bibitem{goyal2017accurate}Goyal, P., Dollár, P., Girshick, R., Noordhuis, P., Wesolowski, L., Kyrola, A., Tulloch, A., Jia, Y. \& He, K. Accurate, large minibatch sgd: Training imagenet in 1 hour. {\em ArXiv Preprint ArXiv:1706.02677}. (2017)
\bibitem{smith2017bayesian}Smith, S. \& Le, Q. A bayesian perspective on generalization and stochastic gradient descent. {\em ArXiv Preprint ArXiv:1710.06451}. (2017)
\bibitem{keskar2016large}Keskar, N., Mudigere, D., Nocedal, J., Smelyanskiy, M. \& Tang, P. On large-batch training for deep learning: Generalization gap and sharp minima. {\em ArXiv Preprint ArXiv:1609.04836}. (2016)
\bibitem{welling2011bayesian}Welling, M. \& Teh, Y. Bayesian learning via stochastic gradient Langevin dynamics. {\em Proceedings Of The 28th International Conference On Machine Learning (ICML-11)}. pp. 681-688 (2011)
\bibitem{zagoruyko2016wide}Zagoruyko, S. \& Komodakis, N. Wide residual networks. {\em ArXiv Preprint ArXiv:1605.07146}. (2016)
\bibitem{zhao2019adaptive}Zhao, R., Vogel, B. \& Ahmed, T. Adaptive Loss Scaling for Mixed Precision Training. {\em ArXiv Preprint ArXiv:1910.12385}. (2019)
\bibitem{krizhevsky2014one}Krizhevsky, A. One weird trick for parallelizing convolutional neural networks. {\em ArXiv Preprint ArXiv:1404.5997}. (2014)
\bibitem{peng2018megdet}Peng, C., Xiao, T., Li, Z., Jiang, Y., Zhang, X., Jia, K., Yu, G. \& Sun, J. Megdet: A large mini-batch object detector. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 6181-6189 (2018)
\bibitem{akiba2017extremely}Akiba, T., Suzuki, S. \& Fukuda, K. Extremely large minibatch sgd: Training resnet-50 on imagenet in 15 minutes. {\em ArXiv Preprint ArXiv:1711.04325}. (2017)
\bibitem{you2019reducing}You, Y., Li, J., Hseu, J., Song, X., Demmel, J. \& Hsieh, C. Reducing BERT pre-training time from 3 days to 76 minutes. {\em ArXiv Preprint ArXiv:1904.00962}. (2019)
\bibitem{you2017imagenet}You, Y., Zhang, Z., Demmel, J., Keutzer, K. \& Hsieh, C. Imagenet training in 24 minutes. {\em ArXiv Preprint ArXiv:1709.05011}. (2017)
\bibitem{lin2017deep}Lin, Y., Han, S., Mao, H., Wang, Y. \& Dally, W. Deep gradient compression: Reducing the communication bandwidth for distributed training. {\em ArXiv Preprint ArXiv:1712.01887}. (2017)
\bibitem{hoffer2017train}Hoffer, E., Hubara, I. \& Soudry, D. Train longer, generalize better: closing the generalization gap in large batch training of neural networks. {\em Advances In Neural Information Processing Systems}. pp. 1731-1741 (2017)
\bibitem{smith2017don}Smith, S., Kindermans, P., Ying, C. \& Le, Q. Don't decay the learning rate, increase the batch size. {\em ArXiv Preprint ArXiv:1711.00489}. (2017)
\bibitem{wu2018group}Wu, Y. \& He, K. Group normalization. {\em Proceedings Of The European Conference On Computer Vision (ECCV)}. pp. 3-19 (2018)
\bibitem{duong-etal-2015}Duong, L., Cohn, T., Bird, S. \& Cook, P. Low Resource Dependency Parsing: Cross-lingual Parameter Sharing in a Neural Network Parser. {\em Proc. Annual Meeting Of The Association For Computational Linguistics And The International Joint Conference On Natural Language Processing}. pp. 845-850 (2015,7)
\bibitem{Caruana1993}Caruana, R. Multitask Learning: A Knowledge-Based Source of Inductive Bias. {\em Proc. International Conference On Machine Learning}. pp. 41-48 (1993)
\bibitem{wang19d}Wang, Z., Zhou, Y., Liang, Y. \& Lan, G. Stochastic Variance-Reduced Cubic Regularization for Nonconvex Optimization. {\em Proc. International Conference On Artificial Intelligence And Statistics (AISTATS)}. \textbf{89} pp. 2731-2740 (2019,4)
\bibitem{zhou2018}Zhou, Y., Wang, Z. \& Liang, Y. Convergence of Cubic Regularization for Nonconvex Optimization under Kundefined Property. {\em Proc. International Conference On Neural Information Processing Systems (NeurIPS)}. pp. 3764-3773 (2018)
\bibitem{nesterov2006}Nesterov, Y. \& Polyak, B. Cubic Regularization of Newton Method and Its Global Performance. {\em Mathematical Programming}. \textbf{108}, 177-205 (2006,8)
\bibitem{Toh2010}Toh, K. \& Yun, S. An Accelerated Proximal Gradient Algorithm for Nuclear Norm Regularized Least Squares Problems. {\em Pacific Journal Of Optimization}. \textbf{6} (2010,9)
\bibitem{candes2012}Candès, E. \& Recht, B. Exact Matrix Completion via Convex Optimization. {\em Communications Of The ACM}. \textbf{55}, 111-119 (2012,6)
\bibitem{Simon2013}Simon, N., Friedman, J., Hastie, T. \& Tibshirani, R. A Sparse-Group Lasso. {\em Journal Of Computational And Graphical Statistics}. \textbf{22}, 231-245 (2013)
\bibitem{Tibshirani2011}Tibshirani, R. Regression shrinkage and selection via the lasso: a retrospective. {\em Journal Of The Royal Statistical Society: Series B (Statistical Methodology)}. \textbf{73}, 273-282 (2011)
\bibitem{Krogh1991}Krogh, A. \& Hertz, J. A Simple Weight Decay Can Improve Generalization. {\em Proc. Advances In Neural Information Processing Systems (NeurIPS)}. pp. 950-957 (1992)
\bibitem{sandler2018mobilenetv2}Sandler, M., Howard, A., Zhu, M., Zhmoginov, A. \& Chen, L. Mobilenetv2: Inverted residuals and linear bottlenecks. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 4510-4520 (2018)
\bibitem{simonyan2014vgg}Simonyan, K. \& Zisserman, A. Very deep convolutional networks for large-scale image recognition. {\em ArXiv Preprint ArXiv:1409.1556}. (2014)
\bibitem{krizhevsky2014cifar}Krizhevsky, A., Nair, V. \& Hinton, G. The cifar-10 dataset. {\em Online: Http://www. Cs. Toronto. Edu/kriz/cifar. Html}. \textbf{55} (2014)
\bibitem{minibatchSGD}Robbins, H. \& Monro, S. A Stochastic Approximation Method. {\em Ann. Math. Statist.}. \textbf{22}, 400-407 (1951,9), https://doi.org/10.1214/aoms/1177729586
\bibitem{fb_largebatch}Goyal, P., Dollár, P., Girshick, R., Noordhuis, P., Wesolowski, L., Kyrola, A., Tulloch, A., Jia, Y. \& He, K. Accurate, Large Minibatch SGD: Training ImageNet in 1 Hour. {\em CoRR}. \textbf{abs/1706.02677} (2017), http://arxiv.org/abs/1706.02677
\bibitem{google_largebatch}Smith, S., Kindermans, P. \& Le, Q. Don't Decay the Learning Rate, Increase the Batch Size. {\em International Conference On Learning Representations}. (2018), https://openreview.net/forum?id=B1Yy1BxCZ
\bibitem{momentumSGD}Sutskever, I., Martens, J., Dahl, G. \& Hinton, G. On the Importance of Initialization and Momentum in Deep Learning. {\em Proceedings Of The 30th International Conference On International Conference On Machine Learning - Volume 28}. pp. III-1139–III–1147 (2013)
\bibitem{largebatch1}Chen, K. \& Huo, Q. Scalable training of deep learning machines by incremental block training with intra-block parallel optimization and blockwise model-update filtering. {\em 2016 IEEE International Conference On Acoustics, Speech And Signal Processing (ICASSP)}. pp. 5880-5884 (2016)
\bibitem{largebatch2}Keskar, N., Mudigere, D., Nocedal, J., Smelyanskiy, M. \& Tang, P. On Large-Batch Training for Deep Learning: Generalization Gap and Sharp Minima. {\em CoRR}. \textbf{abs/1609.04836} (2016), http://arxiv.org/abs/1609.04836
\bibitem{largebatch3}Masters, D. \& Luschi, C. Revisiting Small Batch Training for Deep Neural Networks. {\em CoRR}. \textbf{abs/1804.07612} (2018), http://arxiv.org/abs/1804.07612
\bibitem{lars}You, Y., Gitman, I. \& Ginsburg, B. Scaling SGD Batch Size to 32K for ImageNet Training. {\em CoRR}. \textbf{abs/1708.03888} (2017), http://arxiv.org/abs/1708.03888
\bibitem{anisotropic_noise}Zhu, Z., Wu, J., Yu, B., Wu, L. \& Ma, J. The Anisotropic Noise in Stochastic Gradient Descent: Its Behavior of Escaping from Sharp Minima and Regularization Effects.  (2018)
\bibitem{grover2016node2vec}Grover, A. \& Leskovec, J. node2vec: Scalable feature learning for networks. {\em Proceedings Of The 22nd ACM SIGKDD International Conference On Knowledge Discovery And Data Mining}. pp. 855-864 (2016)
\bibitem{liao2019efficient}Liao, R., Li, Y., Song, Y., Wang, S., Hamilton, W., Duvenaud, D., Urtasun, R. \& Zemel, R. Efficient graph generation with graph recurrent attention networks. {\em Advances In Neural Information Processing Systems}. pp. 4255-4265 (2019)
\bibitem{silver2017mastering}Silver, D., Hubert, T., Schrittwieser, J., Antonoglou, I., Lai, M., Guez, A., Lanctot, M., Sifre, L., Kumaran, D., Graepel, T. \& Others Mastering chess and shogi by self-play with a general reinforcement learning algorithm. {\em ArXiv Preprint ArXiv:1712.01815}. (2017)
\bibitem{wen2019empirical}Wen, Y., Luk, K., Gazeau, M., Zhang, G., Chan, H. \& Ba, J. An Empirical Study of Large-Batch Stochastic Gradient Descent with Structured Covariance Noise.  (2019)
\bibitem{yadavwelcome}Yadav, P., Gupta, M. \& Liptak, V. Welcome Message from SenSys-ML’20 Chairs. 
\bibitem{rotem2018glow}Rotem, N., Fix, J., Abdulrasool, S., Catron, G., Deng, S., Dzhabarov, R., Gibson, N., Hegeman, J., Lele, M., Levenstein, R. \& Others Glow: Graph lowering compiler techniques for neural networks. {\em ArXiv Preprint ArXiv:1805.00907}. (2018)
\bibitem{bleiweiss2008gpu}Bleiweiss, A. GPU accelerated pathfinding. {\em Proceedings Of The 23rd ACM SIGGRAPH/EUROGRAPHICS Symposium On Graphics Hardware}. pp. 65-74 (2008)
\bibitem{gambardella1995ant}Gambardella, L. \& Dorigo, M. Ant-Q: A reinforcement learning approach to the traveling salesman problem. {\em Machine Learning Proceedings 1995}. pp. 252-260 (1995)
\bibitem{karapetyan2017markov}Karapetyan, D., Punnen, A. \& Parkes, A. Markov chain methods for the bipartite boolean quadratic programming problem. {\em European Journal Of Operational Research}. \textbf{260}, 494-506 (2017)
\bibitem{khalil2017learning}Khalil, E., Dai, H., Zhang, Y., Dilkina, B. \& Song, L. Learning combinatorial optimization algorithms over graphs. {\em Advances In Neural Information Processing Systems}. pp. 6348-6358 (2017)
\bibitem{sharafi2015conceptual}Sharafi, P., Teh, L. \& Hadi, M. Conceptual design optimization of rectilinear building frames: A knapsack problem approach. {\em Engineering Optimization}. \textbf{47}, 1303-1323 (2015)
\bibitem{lodi2017learning}Lodi, A. \& Zarpellon, G. On learning and branching: a survey. {\em Top}. \textbf{25}, 207-236 (2017)
\bibitem{chen2019learning}Chen, X. \& Tian, Y. Learning to perform local rewriting for combinatorial optimization. {\em Advances In Neural Information Processing Systems}. pp. 6281-6292 (2019)
\bibitem{nazari2018reinforcement}Nazari, M., Oroojlooy, A., Snyder, L. \& Takác, M. Reinforcement learning for solving the vehicle routing problem. {\em Advances In Neural Information Processing Systems}. pp. 9839-9849 (2018)
\bibitem{burger2020mobile}Burger, B., Maffettone, P., Gusev, V., Aitchison, C., Bai, Y., Wang, X., Li, X., Alston, B., Li, B., Clowes, R. \& Others A Mobile Robotic Chemist. {\em Nature}. \textbf{583}, 237-241 (2020)
\bibitem{martin2018middle}Martin, F., Wang, C., Petty, T., Wang, W. \& Wilkins, P. Middle school students’ social media use. {\em Journal Of Educational Technology & Society}. \textbf{21}, 213-224 (2018)
\bibitem{gleason2018digital}Gleason, B. \& Von Gillern, S. Digital citizenship with social media: Participatory practices of teaching and learning in secondary education. {\em Journal Of Educational Technology & Society}. \textbf{21}, 200-212 (2018)
\bibitem{cappart2019improving}Cappart, Q., Goutierre, E., Bergman, D. \& Rousseau, L. Improving optimization bounds using machine learning: Decision diagrams meet deep reinforcement learning. {\em Proceedings Of The AAAI Conference On Artificial Intelligence}. \textbf{33} pp. 1443-1451 (2019)
\bibitem{song2019co}Song, J., Lanka, R., Yue, Y. \& Ono, M. Co-training for policy learning. {\em ArXiv Preprint ArXiv:1907.04484}. (2019)
\bibitem{junger1995traveling}Jünger, M., Reinelt, G. \& Rinaldi, G. The traveling salesman problem. {\em Handbooks In Operations Research And Management Science}. \textbf{7} pp. 225-330 (1995)
\bibitem{he2014learning}He, H., Daume III, H. \& Eisner, J. Learning to search in branch and bound algorithms. {\em Advances In Neural Information Processing Systems}. pp. 3293-3301 (2014)
\bibitem{vinyals2015pointer}Vinyals, O., Fortunato, M. \& Jaitly, N. Pointer networks. {\em Advances In Neural Information Processing Systems}. pp. 2692-2700 (2015)
\bibitem{hamilton2017inductive}Hamilton, W., Ying, Z. \& Leskovec, J. Inductive representation learning on large graphs. {\em Advances In Neural Information Processing Systems}. pp. 1024-1034 (2017)
\bibitem{sutskever2014sequence}Sutskever, I., Vinyals, O. \& Le, Q. Sequence to sequence learning with neural networks. {\em Advances In Neural Information Processing Systems}. pp. 3104-3112 (2014)
\bibitem{silver2014deterministic}Silver, D., Lever, G., Heess, N., Degris, T., Wierstra, D. \& Riedmiller, M. Deterministic policy gradient algorithms.  (2014)
\bibitem{watkins1992q}Watkins, C. \& Dayan, P. Q-learning. {\em Machine Learning}. \textbf{8}, 279-292 (1992)
\bibitem{yu2020meta}Yu, T., Quillen, D., He, Z., Julian, R., Hausman, K., Finn, C. \& Levine, S. Meta-world: A benchmark and evaluation for multi-task and meta reinforcement learning. {\em Conference On Robot Learning}. pp. 1094-1100 (2020)
\bibitem{rakelly2019efficient}Rakelly, K., Zhou, A., Finn, C., Levine, S. \& Quillen, D. Efficient off-policy meta-reinforcement learning via probabilistic context variables. {\em International Conference On Machine Learning}. pp. 5331-5340 (2019)
\bibitem{gupta2018meta}Gupta, A., Mendonca, R., Liu, Y., Abbeel, P. \& Levine, S. Meta-reinforcement learning of structured exploration strategies. {\em Advances In Neural Information Processing Systems}. pp. 5302-5311 (2018)
\bibitem{kingma2014adam}Kingma, D. \& Ba, J. Adam: A method for stochastic optimization. {\em ArXiv Preprint ArXiv:1412.6980}. (2014)
\bibitem{ruder2016overview}Ruder, S. An overview of gradient descent optimization algorithms. {\em ArXiv Preprint ArXiv:1609.04747}. (2016)
\bibitem{wu2016google}Wu, Y., Schuster, M., Chen, Z., Le, Q., Norouzi, M., Macherey, W., Krikun, M., Cao, Y., Gao, Q., Macherey, K. \& Others Google's neural machine translation system: Bridging the gap between human and machine translation. {\em ArXiv Preprint ArXiv:1609.08144}. (2016)
\bibitem{lpddr4}Assn., J. Low Power Double Data Rate 4 (LPDDR4) Standard. {\em JESD209}. \textbf{4}
\bibitem{hsu2021gptpu}Hsu, K. \& Tseng, H. GPTPU: Accelerating Applications using Edge Tensor Processing Units. {\em ArXiv Preprint ArXiv:2107.05473}. (2021)
\bibitem{kool2018attention}Kool, W., Van Hoof, H. \& Welling, M. Attention, learn to solve routing problems!. {\em ArXiv Preprint ArXiv:1803.08475}. (2018)
\bibitem{zhang2001efficient}Zhang, L., Madigan, C., Moskewicz, M. \& Malik, S. Efficient Conflict Driven Learning in a Boolean Satisfiability Solver. (IEEE Press,2001)
\bibitem{micheli1994synthesis}Micheli, G. Synthesis and Optimization of Digital Circuits. (McGraw-Hill Higher Education,1994)
\bibitem{zhao2015area}Zhao, R., Tan, M., Dai, S. \& Zhang, Z. Area-Efficient Pipelining for FPGA-Targeted High-Level Synthesis. (ACM,2015)
\bibitem{dai2014flushing}Dai, S., Tan, M., Hao, K. \& Zhang, Z. Flushing-Enabled Loop Pipelining for High-Level Synthesis. (ACM,2014)
\bibitem{dai2017dynamic}Dai, S., Zhao, R., Liu, G., Srinath, S., Gupta, U., Batten, C. \& Zhang, Z. Dynamic Hazard Resolution for Pipelining Irregular Loops in High-Level Synthesis. (ACM,2017)
\bibitem{liu2017architecture}Liu, G., Tan, M., Dai, S., Zhao, R. \& Zhang, Z. Architecture and Synthesis for Area-Efficient Pipelining of Irregular Loop Nests. (IEEE,2017)
\bibitem{tan2015elasticflow}Tan, M., Liu, G., Zhao, R., Dai, S. \& Zhang, Z. ElasticFlow: A Complexity-Effective Approach for Pipelining Irregular Loop Nests. (IEEE,2015)
\bibitem{tan2014multithreaded}Tan, M., Liu, B., Dai, S. \& Zhang, Z. Multithreaded Pipeline Synthesis for Data-Parallel Kernels. (IEEE Press,2014)
\bibitem{tan2015mapping}Tan, M., Dai, S., Gupta, U. \& Zhang, Z. Mapping-Aware Constrained Scheduling for LUT-Based FPGAs. (ACM,2015)
\bibitem{ajayi2017celerity}Al, T. Celerity: An Open-Source RISC-V Tiered Accelerator Fabric.  (2017)
\bibitem{ajayi2017experiences}Ajayi, T., Al-Hawaj, K., Amarnath, A., Dai, S., Davidson, S., Gao, P., Liu, G., Rao, A., Rovinski, A., Sun, N., Torng, C., Vega, L., Veluri, B., Xie, S., Zhao, C., Zhao, R., Batten, C., Dreslinski, R., Gupta, R., Taylor, M. \& Zhang, Z. Experiences Using the RISC-V Ecosystem to Design an Accelerator-Centric SoC in TSMC 16nm. {\em First Workshop On Computer Architecture Research With RISC-V (CARRV)}. (2017)
\bibitem{srivastava2017accelerating}Srivastava, N., Dai, S., Manohar, R. \& Zhang, Z. Accelerating Face Detection on Programmable SoC Using C-Based Synthesis.  (2017)
\bibitem{zhou2018rosetta}Zhou, Y., Gupta, U., Dai, S., Zhao, R., Srivastava, N., Jin, H., Featherston, J., Lai, Y., Liu, G., Velasquez, G., Wang, W. \& Zhang, Z. Rosetta: A Realistic Benchmark Suite for Software Programmable FPGAs.  (2018)
\bibitem{liu2016high}Liu, X., Chen, Y., Nguyen, T., Gurumani, S., Rupnow, K. \& Chen, D. High Level Synthesis of Complex Applications: An H.264 Video Decoder. (ACM,2016)
\bibitem{jiang2008scheduling}Jiang, W., Zhang, Z., Potkonjak, M. \& Cong, J. Scheduling with Integer Time Budgeting for Low-Power Optimization. (IEEE Computer Society Press,2008)
\bibitem{dai2017enabling}Dai, S., Liu, G., Zhao, R. \& Zhang, Z. Enabling Adaptive Loop Pipelining in High-Level Synthesis. {\em Asilomar Conf. On Signals, Systems, And Computers}. (2017)
\bibitem{josipovic2017fromc}Josipovic, L., Brisk, P. \& Ienne, P. From C to Elastic Circuits. {\em Asilomar Conf. On Signals, Systems, And Computers}. (2017)
\bibitem{zheng2014fast}Zheng, H., Gurumani, S., Rupnow, K. \& Chen, D. Fast and Effective Placement and Routing Directed High-Level Synthesis for FPGAs. (ACM,2014)
\bibitem{zhang2015high}Zhang, Z., Chen, D., Dai, S. \& Campbell, K. High-Level Synthesis for Low-Power Design. {\em IPSJ Transactions On System LSI Design Methodology (T-SLDM)}. \textbf{8} pp. 12-25 (2015)
\bibitem{cong2010behavior}Cong, J., Liu, B., Majumdar, R. \& Zhang, Z. Behavior-Level Observability Analysis for Operation Gating in Low-Power Behavioral Synthesis. (ACM,2010)
\bibitem{zhang2017high}Zhang, X., Liu, X., Ramachandran, A., Zhuge, C., Tang, S., Ouyang, P., Cheng, Z., Rupnow, K. \& Chen, D. High-Performance Video Content Recognition with Long-Term Recurrent Convolutional Network for FPGA. (IEEE,2017)
\bibitem{zhao2017accelerating}Zhao, R., Song, W., Zhang, W., Xing, T., Lin, J., Srivastava, M., Gupta, R. \& Zhang, Z. Accelerating Binarized Convolutional Neural Networks with Software-Programmable FPGAs. {\em FPGA}. pp. 15-24 (2017)
\bibitem{liang2012high}Liang, Y., Rupnow, K., Li, Y., Min, D., Do, M. \& Chen, D. High-Level Synthesis: Productivity, Performance, and Software Constraints. {\em Journal Of Electrical And Computer Engineering}. \textbf{2012} pp. 1 (2012)
\bibitem{liu2015offline}Liu, J., Bayliss, S. \& Constantinides, G. Offline Synthesis of Online Dependence Testing: Parametric Loop Pipelining for HLS. (IEEE,2015)
\bibitem{alle2013runtime}Alle, M., Morvan, A. \& Derrien, S. Runtime Dependency Analysis for Loop Pipelining in High-Level Synthesis. (ACM,2013)
\bibitem{rau1996iterative}Rau, B. Iterative Modulo Scheduling. {\em International Journal Of Parallel Programming}. \textbf{24}, 3-64 (1996)
\bibitem{canis2014modulo}Canis, A., Brown, S. \& Anderson, J. Modulo SDC Scheduling with Recurrence Minimization in High-Level Synthesis. (IEEE,2014)
\bibitem{zhang2013sdc}Zhang, Z. \& Liu, B. SDC-Based Modulo Scheduling for Pipeline Synthesis. (IEEE Press,2013)
\bibitem{hara2008chstone}Hara, Y., Tomiyama, H., Honda, S., Takada, H. \& Ishii, K. CHStone: A Benchmark Program Suite for Practical C-Based High-Level Synthesis. (IEEE,2008)
\bibitem{marques2008practical}Marques-Silva, J. Practical Applications of Boolean Satisfiability. {\em Int'l Workshop On Discrete Event Systems (WODES)}. pp. 74-80 (2008)
\bibitem{stallman1999using}Stallman, R. Using and Porting the GNU Compiler Collection. {\em Free Software Foundation}. \textbf{86} (1999)
\bibitem{czajkowski2012opencl}Czajkowski, T., Neto, D., Kinsner, M., Aydonat, U., Wong, J., Denisenko, D., Yiannacouras, P., Freeman, J., Singh, D. \& Brown, S. OpenCL for FPGAs: Prototyping a Compiler. {\em Int'l Conf. On Engineering Of Reconfigurable Systems And Algorithms (ERSA)}. pp. 1 (2012)
\bibitem{nieuwenhuis2012sat}Nieuwenhuis, R. SAT and SMT are Still Resolution: Questions and Challenges. {\em Automated Reasoning}. pp. 10-13 (2012)
\bibitem{de2008z3}De Moura, L. \& Bjørner, N. Z3: An Efficient SMT Solver. {\em Tools And Algorithms For The Construction And Analysis Of Systems}. pp. 337-340 (2008)
\bibitem{dutertre2014yices}Dutertre, B. Yices 2.2. {\em Int'l Conf. On Computer Aided Verification (CAV)}. pp. 737-744 (2014)
\bibitem{barrett2011cvc4}Barrett, C., Conway, C., Deters, M., Hadarean, L., Jovanović, D., King, T., Reynolds, A. \& Tinelli, C. CVC4. {\em Int'l Conf. On Computer Aided Verification (CAV)}. pp. 171-177 (2011)
\bibitem{chen2013branch}Chen, M., Huang, S., Pu, G. \& Mishra, P. Branch-and-Bound Style Resource Constrained Scheduling using Efficient Structure-Aware Pruning. {\em IEEE Computer Society Annual Symposium On VLSI (ISVLSI)}. pp. 224-229 (2013)
\bibitem{yu2010place}Yu, C., Wu, Y. \& Wang, S. An In-Place Search Algorithm for the Resource Constrained Scheduling Problem during High-Level Synthesis. (ACM,2010)
\bibitem{wang2005deciding}Wang, C., Ivančić, F., Ganai, M. \& Gupta, A. Deciding Separation Logic Formulae by SAT and Incremental Negative Cycle Elimination. {\em Logic For Programming, Artificial Intelligence, And Reasoning}. pp. 322-336 (2005)
\bibitem{cotton2005satisfiability}Cotton, S., Podelski, A. \& Finkbeiner, B. Satisfiability Checking with Difference Constraints. {\em Int'l Max Planck Research School For Computer Science, Saarbrüceken,Germany}. (2005)
\bibitem{narasimhan2001fast}Narasimhan, M. \& Ramanujam, J. A Fast Approach to Computing Exact Solutions to the Resource-Constrained Scheduling Problem. (ACM,2001)
\bibitem{cbc2005}Forrest, J. CBC User Guide. {\em IBM Research}. \textbf{46}, 157 (2005)
\bibitem{cplex2009v126}CPLEX, I. V12.6: User`s Manual for CPLEX. {\em International Business Machines Corporation}. \textbf{46}, 157 (2015)
\bibitem{biere2013lingeling}Biere, A. Lingeling, Plingeling and Treengeling Entering the SAT Competition 2013. {\em SAT Competition}. \textbf{2013} (2013)
\bibitem{LaAd04:LLVM}Lattner, C. \& Adve, V. LLVM: a Compilation Framework for Lifelong Program Analysis & Transformation.  (2004,3)
\bibitem{chinneck1991locating}Chinneck, J. \& Dravnieks, E. Locating Minimal Infeasible Constraint Sets in Linear Programs. {\em ORSA Journal On Computing}. \textbf{3}, 157-168 (1991)
\bibitem{rim1994lower}Rim, M. \& Jain, R. Lower-bound Performance Estimation for the High-Level Synthesis Scheduling Problem. (IEEE,1994)
\bibitem{ramalingam1999solving}Ramalingam, G., Song, J., Joskowicz, L. \& Miller, R. Solving Systems of Difference Constraints Incrementally. {\em Algorithmica}. \textbf{23}, 261-275 (1999)
\bibitem{van1981irreducibly}Van Loon, J. Irreducibly Inconsistent Systems of Linear Inequalities. {\em European Journal Of Operational Research}. \textbf{8}, 283-288 (1981)
\bibitem{pratt1977two}Pratt, V. Two Easy Theories whose Combination is Hard. (Massachusetts Institute of Technology,1977)
\bibitem{horbach2010boolean}Horbach, A. A Boolean Satisfiability Approach to the Resource-Constrained Project Scheduling Problem. {\em Annals Of Operations Research}. \textbf{181}, 89-107 (2010)
\bibitem{malik2009boolean}Malik, S. \& Zhang, L. Boolean Satisfiability from Theoretical Hardness to Practical Success. {\em Communications Of The ACM}. \textbf{52}, 76-82 (2009)
\bibitem{davis1962machine}Davis, M., Logemann, G. \& Loveland, D. A Machine Program for Theorem-Proving. {\em Communications Of The ACM}. \textbf{5}, 394-397 (1962)
\bibitem{de2011satisfiability}De Moura, L. \& Bjørner, N. Satisfiability Modulo Theories: Introduction and Applications. {\em Communications Of The ACM}. \textbf{54}, 69-77 (2011)
\bibitem{CoZh06:sdc}Cong, J. \& Zhang, Z. An Efficient and Versatile Scheduling Algorithm Based on SDC Formulation.  (2006)
\bibitem{parker1986maha}Parker, A., Pizarro, J. \& Mlinar, M. MAHA: A Program for Datapath Synthesis. (IEEE Press,1986)
\bibitem{canis2011legup}Al., A. LegUp: High-Level Synthesis for FPGA-Based Processor/Accelerator Systems.  (2011)
\bibitem{CoLi11:autoesl}Cong, J., Liu, B., Neuendorffer, S., Noguera, J., Vissers, K. \& Zhang, Z. High-Level Synthesis for FPGAs: From Prototyping to Deployment.  (2011)
\bibitem{ratner2019sysml}Ratner, A., Alistarh, D., Alonso, G., Bailis, P., Bird, S., Carlini, N., Catanzaro, B., Chung, E., Dally, B., Dean, J. \& Others SysML: The New Frontier of Machine Learning Systems. {\em ArXiv Preprint ArXiv:1904.03257}. (2019)
\bibitem{paulin1989force}Paulin, P. \& Knight, J. Force-directed scheduling for the behavioral synthesis of ASICs. {\em IEEE Transactions On Computer-Aided Design Of Integrated Circuits And Systems}. \textbf{8}, 661-679 (1989)
\bibitem{yang1993list}Yang, T. \& Gerasoulis, A. List scheduling with and without communication delays. {\em Parallel Computing}. \textbf{19}, 1321-1344 (1993)
\bibitem{ahn2020ordering}Ahn, B., Lee, J., Lin, J., Cheng, H., Hou, J. \& Esmaeilzadeh, H. Ordering chaos: Memory-aware scheduling of irregularly wired neural networks for edge devices. {\em ArXiv Preprint ArXiv:2003.02369}. (2020)
\bibitem{leiserson1991retiming}Leiserson, C. \& Saxe, J. Retiming synchronous circuitry. {\em Algorithmica}. \textbf{6}, 5-35 (1991)

\end{thebibliography}

==> figures/exploration_figures.tex <==
\begin{figure}[!htb]
\centering
% ROW 1 1
\iffalse
\begin{minipage}{0.46\textwidth}
  \centering
 \includegraphics[width=0.7\textwidth]{./figures/undersize-mismatch.pdf}
\subcaption{TBD}\label{fig:graph_complexity_mismatch}
\end{minipage}
\fi
% ROW 1 2

\begin{minipage}{0.45\textwidth}
  \centering
 %\includegraphics[width=1\textwidth]{./figures/oversize-6-mismatch.pdf}
 \includegraphics[width=0.7\textwidth]{./figures/oversize-6-mismatch-crop.pdf}
\subcaption{Testing mismatch with different training graph in-degree constrains $deg(V)$=\{3,4,5,6\}}\label{fig:graph_complexity_mismatch}
\end{minipage}
% ROW 1 3
\hspace{5mm}
\begin{minipage}{0.45\textwidth}
  \centering
 \includegraphics[width=0.7\textwidth]{./figures/oversize-6-loss.pdf}
\subcaption{Testing loss while training with different graph in-degree constrains $deg(V)$=\{3,4,5,6\}}\label{fig:graph_complexity_loss}
\end{minipage}

\iffalse
\begin{figure}
    \centering
     \begin{subfigure}[b]{0.3\linewidth}
         \centering
         \includegraphics[width=0.7\textwidth]{./figures/oversize-6-mismatch-crop.pdf}
         \caption{Testing mismatch while training with different graph in-degree constrains $deg(V)$=\{3,4,5,6\}}
         \label{fig:graph_complexity_mismatch}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=0.7\textwidth]{./figures/scheduling-direction-mismatch-crop.pdf}
        \caption{Testing mismatch comparisons  between training with ASAP and ALAP scheduling as targeted labels}
        \label{fig:directional_explore_mismatch}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=0.7\textwidth]{./figures/toposort30_50_misMatch_6inDegree_encoder_decoder_type_comparison_1e-6-crop.pdf}
        \caption{Testing mismatch with four different configurations of PtrNet (lr=$10^{-6}$)}
        \label{fig:ptr_explore_mismatch}
     \end{subfigure}
        \caption{}
        \label{fig:three graphs}
\end{figure}
\fi

% Row 2 2
\begin{minipage}{0.4\textwidth}
  \centering
 %\includegraphics[width=1\textwidth]{./figures/scheduling-direction-mismatch.pdf}
 \includegraphics[width=0.7\textwidth]{./figures/scheduling-direction-mismatch-crop.pdf}
\subcaption{Testing mismatch comparisons  between training with ASAP and ALAP scheduling as targeted labels}\label{fig:directional_explore_mismatch}
\end{minipage}
% ROW 2 3
\hspace{5mm}
\begin{minipage}{0.4\textwidth}
  \centering
 \includegraphics[width=0.7\textwidth]{./figures/scheduling-direction-loss.pdf}
\subcaption{Testing loss comparisons  between training with ASAP and ALAP scheduling as targeted labels}\label{fig:directional_explore_loss}
\end{minipage}
\begin{minipage}{0.46\textwidth}
  \centering
%\includegraphics[width=1\textwidth]{./figures/mismatch_encoder_decoder.pdf}
 \includegraphics[width=0.7\textwidth]{./figures/toposort30_50_misMatch_6inDegree_encoder_decoder_type_comparison_1e-6-crop.pdf}
\subcaption{Testing mismatch with four different configurations of PtrNet (lr=$10^{-6}$)}\label{fig:ptr_explore_mismatch}
\end{minipage}
%
\hspace{5mm}
\begin{minipage}{0.4\textwidth}
  \centering
\includegraphics[width=1\textwidth]{./figures/loss_encoder_decoder.pdf}
\subcaption{Testing loss with four different configurations of PtrNet (lr=$10^{-6}$)}\label{fig:ptr_explore_loss}
\end{minipage}
\caption{Explorations of training setups and neural architecture configurations by measuring the testing performance using \texttt{mismatch} and loss values, specifically covering aspects of training graphs complexity, scheduling types, and encoder-decoder architectures.}
\label{fig:exploration}
\end{figure}

==> figures/subfigure.tex <==
\iffalse
\begin{figure*}
    \centering
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{./figures/oversize-6-mismatch-crop.pdf}
         \caption{Testing mismatch while training with different graph in-degree constrains $deg(V)$=\{3,4,5,6\}}
         \label{fig:graph_complexity_mismatch}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{./figures/scheduling-direction-mismatch-crop.pdf}
        \caption{Testing mismatch comparisons  between training with ASAP and ALAP scheduling as targeted labels}
        \label{fig:directional_explore_mismatch}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{./figures/toposort30_50_misMatch_6inDegree_encoder_decoder_type_comparison_1e-6-crop.pdf}
        \caption{Testing mismatch with four different configurations of PtrNet (lr=$10^{-6}$)}
        \label{fig:ptr_explore_mismatch}
     \end{subfigure}
    
    \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{./figures/oversize-6-loss.pdf}
        \caption{Testing loss while training with different graph in-degree constrains $deg(V)$=\{3,4,5,6\}}
        \label{fig:graph_complexity_loss}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=1\linewidth]{./figures/scheduling-direction-loss.pdf}
        \caption{Testing mismatch comparisons  between training with ASAP and ALAP scheduling as targeted labels}
        \label{fig:directional_explore_loss}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=1\textwidth]{./figures/loss_encoder_decoder.pdf}
        \caption{Testing loss with four different configurations of PtrNet (lr=$10^{-6}$)}\label{fig:ptr_explore_loss}
     \end{subfigure}
     
    \caption{Explorations of training setups and neural architecture configurations by measuring the testing performance using \texttt{mismatch} and loss values, specifically covering aspects of training graphs complexity, scheduling types, and encoder-decoder architectures.}
\label{fig:exploration}
\end{figure*}
\fi

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figures/speedup.pdf}
    \caption{\color{red}Caption}
    \label{fig:scheduling_overhead}
\end{figure*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

